Emoji-Powered Representation Learning for Cross-Lingual Sentiment Classification

Sentiment classification typically relies on a large amount of labeled data. In practice, the availability of labels is highly imbalanced among different languages, e.g., more English texts are labeled than texts in any other languages, which creates a considerable inequality in the quality of related information services received by users speaking different languages. To tackle this problem, cross-lingual sentiment classification approaches aim to transfer knowledge learned from one language that has abundant labeled examples (i.e., the source language, usually English) to another language with fewer labels (i.e., the target language). The source and the target languages are usually bridged through off-the-shelf machine translation tools. Through such a channel, cross-language sentiment patterns can be successfully learned from English and transferred into the target languages. This approach, however, often fails to capture sentiment knowledge specific to the target language, and thus compromises the accuracy of the downstream classification task. In this paper, we employ emojis, which are widely available in many languages, as a new channel to learn both the cross-language and the language-specific sentiment patterns. We propose a novel representation learning method that uses emoji prediction as an instrument to learn respective sentiment-aware representations for each language. The learned representations are then integrated to facilitate cross-lingual sentiment classification. The proposed method demonstrates state-of-the-art performance on benchmark datasets, which is sustained even when sentiment labels are scarce.

==> section/limitation.tex <==
\section{Limitations}\label{limitation}
%As we have demonstrated the encouraging performance of our approach, then we want to discuss the implications of our study and some threads to our evaluation.
%
%\subsection{Limitations}\label{limitation}
Next, we discuss some limitations or threats to validity in our evaluations.

%\para{Generalizability}
%Currently, we have evaluated our cross-lingual sentiment classification approach on Amazon reviews and Tweets. However, even some popular and well evaluated sentiment analysis approaches are demonstrated to have poor performance on data sets with specific domain knowledge such as software engineering tasks~\cite{BinLin18}. In the future, we plan to apply our approach on more various tasks and further evaluate the generalization. 

\para{Tokenizer and Translation Tool}
Indeed, our approach relies on the existing tools such as \textit{MeCab} and \textit{Google Translate}. Although these tools are widely adopted in previous work, they still may not perform perfectly and thus can affect our classification performance. As tokenizing and translation are also hot research topics in natural language processing, we can apply alternative effective tools in future work to alleviate this limitation.

\para{Diverse Emoji Usage}
Emojis have been demonstrated to have various non-verbal functions, such as expressing sentiment, adjust tones, or express irony. For different usage purposes, emojis sometimes are used in sentiments with opposite sentiments~\cite{HuGSNL17}. The habits of emoji usage are influenced by cultures~\cite{Lu16}, gender~\cite{zhenpeng18}, age~\cite{ZhouHK17}, platforms~\cite{MillerTCJTH16,MillerKTTH17}, etc. Although expressing sentiment is the most used function~\cite{HuGSNL17}, the uncertain and various emoji usage still leads to noise in distant-supervised phase~\cite{yuxiao2018}. 
%In future work, we plan to train a classification of emoji usage purposes and filter out the emoji-texts in which emojis are not the proxies of sentiments to further improve the performance. 


%\subsection{Implications}
%In ubiquitous computing community, user-generated texts such as Tweets have been considered as a special passive ``sensor'' of users' sentiments and emotions~\cite{SahaCBAC17}. Compared to the active sensors such as ecological momentary assessment (EMA)~\cite{csikszentmihalyi2014validity} and traditional passive sensors such as wearable sensors~\cite{AdamsRRMVGCV14}, using texts to infer sentiment is less costly and easier to scale. However, due to the research ``inequality'' among languages, this convenient ``sensor'' technique is absent in many non-English languages. Yet the urgent demand in these according non-English countries to it is never absent. 
%For example, it was reported in some non-English countries such as Japan, mental health concerns are quite serious~\cite{kanata2016japanese}, which calls for an efficient approach to sensing and detecting the disorders of users' emotional states. The text-based sentiment analysis exactly serves this need. For one thing, users tend to generate texts frequently in daily life, which lays a solid foundation for us to sense their sentiment instability accurately and timely. For another, text-based sentiment analysis shows its unique advantages in passive and effortless sensing. Considering the lack of text-based sentiment research in these non-English languages and its obvious advantages, our cross-lingual sentiment analysis can have potential effects and the preliminary results may shed new light on this area.
%
%We want to further discuss the insights of emojis, since they exactly play an important role in our approach. As a new ubiquitous language, emojis are widely adopted across the world~\cite{Lu16}, attracting a lot of researchers to study their usage patterns~\cite{Lu16,zhenpeng18,ZhouHK17} and non-verbal functions~\cite{HuGSNL17,CramerJT16,tochi/PohlDR17}. These empirical findings lead us to move a step further to expand emoji's abilities as a novel ``sensor" in the real world. Based on the previous findings that emojis are widely used to express sentiment across languages~\cite{Lu16,HuGSNL17}, in this study, we explore this ``sensor"  ability of emoji from an sentiment probing perspective. More specifically, our study exploits emojis' ubiquitous and emotional characteristic in diverse languages directly considering emojis as weak sentiment labels and shows promising results. Our successful attempt can in turn encourage the researchers in ubiquitous computing and human-computer interaction community to excavate the ``sensor"  ability of emoji to user profiles, with their abundant findings of emoji usage differences across cultures~\cite{Lu16}, ages~\cite{ZhouHK17}, genders~\cite{zhenpeng18} and so on. Considering the similar ``research inequality'' in user profiling~\cite{CiotSR13} (i.e., the existing text-based user profiling studies mainly focus on English users), using ubiquitous emojis to infer the background, gender, age of users can be generalized to diverse languages and thus narrows the current research gap.
